DisCoPy: Monoidal Categories in Python

We introduce DisCoPy, an open source toolbox for computing with monoidal categories. The library provides an intuitive syntax for defining string diagrams and monoidal functors. Its modularity allows the efficient implementation of computational experiments in the various applications of category theory where diagrams have become a lingua franca. As an example, we used DisCoPy to perform natural language processing on quantum hardware for the first time.

==> eptcsdata.tex <==
\providecommand{\firstpage}{183}
\providecommand{\publicationstatus}{David I. Spivak and Jamie Vicary (Eds.):\\
Applied Category Theory 2020 (ACT2020)\\
EPTCS 333, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.333.13}{10.4204/EPTCS.333.13}}


==> header.tex <==
%!TEX root = ms.tex

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}

\RequirePackage{doi}
\usepackage{hyperref}

\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{newtxtext, newtxmath}
\usepackage{braket}
\usepackage{physics}
\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{matrix,arrows,decorations.pathmorphing}
\usetikzlibrary{decorations.markings}

\usepackage{pgfplots}
\DeclareUnicodeCharacter{2212}{−}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}

\newcommand{\s}{\enspace}
\newcommand{\sub}{\subseteq}
\newcommand{\size}[1]{\left\vert{#1}\right\vert}
\renewcommand{\cal}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\phi}{\varphi}
\newcommand{\xto}[1]{\xrightarrow{#1}}
\newcommand{\injects}{\xhookrightarrow{}}
\newcommand{\from}{\leftarrow}
\newcommand{\rel}[3]{#1 \sub #2 \times #3}
\newcommand{\graph}[2]{#1 \sub #2^2}
\newcommand{\B}{\bb{B}}
\newcommand{\N}{\bb{N}}
\newcommand{\Z}{\bb{Z}}

\newtheorem{draft}{DRAFT}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{conjecture}[definition]{Conjecture}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{example}[definition]{Example}
\newtheorem{remark}[definition]{Remark}
\newtheorem*{class}{class}
\newtheorem*{method}{method}

\usepackage{xpatch}
\makeatletter
\AtBeginDocument{\xpatchcmd{\@thm}{\thm@headpunct{.}}{\thm@headpunct{}}{}{}}
\makeatother

\setlength{\fboxsep}{2pt}
\setlength{\fboxrule}{0.1pt}
\newcommand{\py}[1]{{\color{gray}\fbox{\raisebox{0pt}[8pt][2pt]{\color{brown}\normalfont\texttt{#1}}}}}

\usepackage{pythonhighlight}

\usepackage[linesnumbered,boxed,noend]{algorithm2e}

